Comparing Personalized Relevance Algorithms for Directed Graphs

We present an interactive Web platform that, given a directed graph, allows identifying the most relevant nodes related to a given query node. Besides well-established algorithms such as PageRank and Personalized PageRank, the demo includes Cyclerank, a novel algorithm that addresses some of their limitations by leveraging cyclic paths to compute personalized relevance scores. Our demo design enables two use cases: (a) algorithm comparison, comparing the results obtained with different algorithms, and (b) dataset comparison, for exploring and gaining insights into a dataset and comparing it with others. We provide 50 pre-loaded datasets from Wikipedia, Twitter, and Amazon and seven algorithms. Users can upload new datasets, and new algorithms can be easily added. By showcasing efficient algorithms to compute relevance scores in directed graphs, our tool helps to uncover hidden relationships within the data, which makes of it a valuable addition to the repertoire of graph analysis algorithms.

==> tables/comparison_amazon-cr5-pr0_85-ssppr0_85-top5.tex <==
\resizebox{.95\textwidth}{!}{
\begin{tabular}{@{}rp{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}@{}}
  \toprule
    \textbf{page}
  & \multicolumn{2}{c}{\thead{\bfseries 1984}}%
  & \multicolumn{2}{c}{\thead{\bfseries The Fellowship of the Ring}}%
  & \multicolumn{2}{c}{\thead{\bfseries Blade Runner}}%
  \\ %
  \cmidrule(l){2-3}%
  \cmidrule(l){4-5}%
  \cmidrule(l){6-7}%
  %
    \textbf{\#}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  \\%
  1  & Animal Farm                                  & The Catcher in the Rye                             %
     & The Hobbit                                   & The Silmarillion                                   %
     & Dark City                                    & 2001 - A Space Odyssey                             %
     \\%
  2  & Fahrenheit 451                               & Lord of the Flies                                  %
     & The Return of the King                       & The Hobbit                                         %
     & 2001 - A Space Odyssey                       & Dark City                                          %
     \\%
  3  & The Catcher in the Rye                       & Animal Farm                                        %
     & The Silmarillion                             & \makecell[tl]{Harry Potter and the\\%
                                                                    Sorcerer's Stone}                    %
     & Gattaca                                      & Donnie Darko                                       %
     \\%
  4  & Brave New World                              & Fahrenheit 451                                     %
     & The Two Towers                               & \makecell[tl]{Harry Potter and the\\%
                                                                    Chamber of Secrets}                  %
     & \makecell[tl]{The City of Lost\\
                     Children}                      & Requiem for a Dream                                %
     \\%
  5  & Lord of the Flies                            & To Kill a Mockingbird                              %
     & Unfinished Tales .. .                        & The Return of the King                             %
     & eXistenZ                                     & A Clockwork Orange                                 %
     \\%
  \bottomrule
\end{tabular}%
}

% ---
% Parameters:
% Algorihtm   Cyclerank
% Dataset  amazon-meta.labeled.txt
% Source   [Book][ASIN: 0451524934] 1984
% maxloop  5
% scoring_function  exp
%
% Ranking:
%    ID Label Score
% #1 449223   [Book][ASIN: 0451524934] 1984 2.151
% #2 53175 [Book][ASIN: 0451526341] Animal Farm   1.071
% #3 29543 [Book][ASIN: 0345342968] Fahrenheit 451   0.994
% #4 98756 [Book][ASIN: 0316769487] The Catcher in the Rye 0.978
% #5 353397   [Book][ASIN: 0060929871] Brave New World  0.747
% #6 35512 [Book][ASIN: 0399501487] Lord of the Flies   0.629
% #7 537519   [Book][ASIN: 0446310786] To Kill a Mockingbird  0.391
% #8 341570   [Book][ASIN: 0140177396] Of Mice and Men (Penguin Great Books of the 20th Century)  0.190
% #9 517948   [Book][ASIN: 0440180295] Slaughterhouse-Five 0.170
% #10   449014   [Book][ASIN: 0764585975] Golding's the Lord of the Flies (Cliffs Notes) 0.065
% #11   308339   [Book][ASIN: 0764585851] 1984 (Cliffs Notes) 0.04
%
% Parameters:
% Algorihtm   Single Source Personalized PageRank
% Dataset  amazon-meta.labeled.txt
% Source   [Book][ASIN: 0451524934] 1984
% alpha 0.85
%
% Ranking:
%    ID Label Score
% #1 449223   [Book][ASIN: 0451524934] 1984 0.214
% #2 98756 [Book][ASIN: 0316769487] The Catcher in the Rye 0.131
% #3 35512 [Book][ASIN: 0399501487] Lord of the Flies   0.118
% #4 53175 [Book][ASIN: 0451526341] Animal Farm   0.101
% #5 29543 [Book][ASIN: 0345342968] Fahrenheit 451   0.077
% #6 537519   [Book][ASIN: 0446310786] To Kill a Mockingbird  0.076
% #7 341570   [Book][ASIN: 0140177396] Of Mice and Men (Penguin Great Books of the 20th Century)  0.059
% #8 353397   [Book][ASIN: 0060929871] Brave New World  0.050
% #9 199628   [Book][ASIN: 0684801523] The Great Gatsby 0.032
% #10   449014   [Book][ASIN: 0764585975] Golding's the Lord of the Flies (Cliffs Notes) 0.023
% #11   211438   [Book][ASIN: 0142000663] The Grapes of Wrath : (Centennial Edition)  0.01
%
%---
%
% Parameters:
% Algorihtm   Cyclerank
% Dataset  amazon-meta.labeled.txt
% Source   [Book][ASIN: 0788789813] The Fellowship of the Ring (The Lord of the Rings, Book 1)
% maxloop  5
% scoring_function  exp
%
% Ranking:
%    ID Label Score
% #1 78057 [Book][ASIN: 0788789813] The Fellowship of the Ring (The Lord of the Rings, Book 1) 0.557
% #2 392323   [Book][ASIN: 0395177111] The Hobbit (Leatherette Collector's Edition)   0.421
% #3 473049   [Book][ASIN: 0788789848] The Return of the King (The Lord of the Rings, Book 3)  0.297
% #4 75863 [Book][ASIN: 0345325818] The Silmarillion 0.118
% #5 251356   [Book][ASIN: 078878983X] The Two Towers (The Lord of the Rings, Book 2) 0.093
% #6 88616 [Book][ASIN: 0345357116] Unfinished Tales: The Lost Lore of Middle-earth   0.007
%
%---
% Parameters:
% Algorihtm   Single Source Personalized PageRank
% Dataset  amazon-meta.labeled.txt
% Source   [Book][ASIN: 0788789813] The Fellowship of the Ring (The Lord of the Rings, Book 1)
% alpha 0.85
%
% Ranking:
%    ID Label Score
% #1 78057 [Book][ASIN: 0788789813] The Fellowship of the Ring (The Lord of the Rings, Book 1) 0.178
% #2 75863 [Book][ASIN: 0345325818] The Silmarillion 0.088
% #3 392323   [Book][ASIN: 0395177111] The Hobbit (Leatherette Collector's Edition)   0.072
% #4 526761   [Book][ASIN: 0590353403] Harry Potter and the Sorcerer's Stone (Book 1) 0.054
% #5 216201   [Book][ASIN: 0439064864] Harry Potter and the Chamber of Secrets (Book 2)  0.051
% #6 473049   [Book][ASIN: 0788789848] The Return of the King (The Lord of the Rings, Book 3)  0.046
% #7 88616 [Book][ASIN: 0345357116] Unfinished Tales: The Lost Lore of Middle-earth   0.039
% #8 429348   [Book][ASIN: 043935806X] Harry Potter and the Order of the Phoenix (Book 5)   0.038
% #9 404634   [Book][ASIN: 0439136350] Harry Potter and the Prisoner of Azkaban (Book 3) 0.035
% #10   115022   [Book][ASIN: 0345375211] The Book of Lost Tales, Part One (The History of Middle-Earth, Vol. 1) 0.033
% #11   251356   [Book][ASIN: 078878983X] The Two Towers (The Lord of the Rings, Book 2) 0.030
%
% ---
% Parameters:
% Algorihtm   Cyclerank
% Dataset  amazon-meta.labeled.txt
% Source   [DVD][ASIN: 0790729628] Blade Runner (The Director's Cut)
% maxloop  5
% scoring_function  exp
%
% Ranking:
%    ID Label Score
% #1 545235   [DVD][ASIN: 0790729628] Blade Runner (The Director's Cut)   0.495
% #2 544653   [DVD][ASIN: 0780622553] Dark City (New Line Platinum Series)   0.285
% #3 83709 [DVD][ASIN: B00005ASUM] 2001 - A Space Odyssey  0.210
% #4 175372   [DVD][ASIN: 0767805712] Gattaca  0.075
% #5 54534 [DVD][ASIN: B00000K3TS] The City of Lost Children  0.068
% #6 18833 [DVD][ASIN: B00000K31V] eXistenZ 0.032
% #7 166709   [DVD][ASIN: B00003CX9G] Close Encounters of the Third Kind (Two-Disc Collector's Edition) 0.025
% #8 139429   [DVD][ASIN: 0780022181] Brazil - Criterion Collection 0.018
% #9 547536   [DVD][ASIN: 0767821629] The Thirteenth Floor 0.013
% #10   262143   [DVD][ASIN: 0790733226] Contact  0.007
%
% ---
% Parameters:
% Algorihtm   Single Source Personalized PageRank
% Dataset  amazon-meta.labeled.txt
% Source   [DVD][ASIN: 0790729628] Blade Runner (The Director's Cut)
% alpha 0.85
%
% Ranking:
%    ID Label Score
% #1 545235   [DVD][ASIN: 0790729628] Blade Runner (The Director's Cut)   0.200
% #2 83709 [DVD][ASIN: B00005ASUM] 2001 - A Space Odyssey  0.108
% #3 544653   [DVD][ASIN: 0780622553] Dark City (New Line Platinum Series)   0.102
% #4 546221   [DVD][ASIN: B00005V3Z4] Donnie Darko   0.034
% #5 547638   [DVD][ASIN: B00005Q4CS] Requiem for a Dream (Director's Cut)   0.033
% #6 184382   [DVD][ASIN: B00005ATQB] A Clockwork Orange   0.028
% #7 166709   [DVD][ASIN: B00003CX9G] Close Encounters of the Third Kind (Two-Disc Collector's Edition) 0.028
% #8 18833 [DVD][ASIN: B00000K31V] eXistenZ 0.025
% #9 545523   [DVD][ASIN: B00004VVN8] 2010: The Year We Make Contact   0.025
% #10   175372   [DVD][ASIN: 0767805712] Gattaca  0.025
% #11   235687   [DVD][ASIN: B000055Y0X] Dr. Strangelove or How I Learned to Stop Worrying and Love the Bomb (Special Edition)  0.025

==> tables/comparison_wikipedia-cr3-pr0_3-ssppr0_3-top5.tex <==
\resizebox{.95\textwidth}{!}{
\begin{tabular}{@{}rp{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}@{}}
  \toprule
    \textbf{page}
  & \multicolumn{2}{c}{\thead{\bfseries Internet}}%
  & \multicolumn{2}{c}{\thead{\bfseries Freddie Mercury}}%
  & \multicolumn{2}{c}{\thead{\bfseries Pasta}}%
  \\ %
  \cmidrule(l){2-3}%
  \cmidrule(l){4-5}%
  \cmidrule(l){6-7}%
  %
    \textbf{\#}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  \\%
  1  & \makecell[tl]{Index of Internet-related\\%
                   articles}                        & Voice over IP                                      %
     & Queen (band)                                 & Queen (band)                                       %
     & Italian cuisine                              & Bolognese sauce                                    %
     \\%
  2  & Computer network                             & Internet protocol suite                            %
     & Brian May                                    & \makecell[tl]{The Freddie Mercury\\%
                                                                  Tribute Concert}                       %
     & Italy                                        & Carbonara                                          %
     \\%
  3  & Facebook                                     & Internet forum                                     %
     & \makecell[tl]{Roger Taylor\\%
                   (Queen drummer)}                 & HIV/AIDS                                           %
     & Spaghetti                                    & Durum                                              %
     \\%
  4  & World Wide Web                               & Internet access                                    %
     & John Deacon                                  & Queen II                                           %
     & Flour                                        & Italy                                              %
     \\%
  5  & Google                                       & Internet service provider                          %
     & Made in Heaven                               & Mercury Phoenix Trust                              %
     & Durum                                        & United States                                      %
     \\%
  \bottomrule
\end{tabular}%
}

% ---
% Parameters
% Algorihtm   Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Internet
% maxloop  3
% scoring_function  exp
%
% Ranking
%    ID Label Score
% #0 9167  Internet 298.056
% #1 151847   Index of Internet-related articles  7.852
% #2 1705417  Computer network  6.558
% #3 2614687  Facebook 5.911
% #4 21479 World Wide Web 5.562
% #5 611580   Google   5.512
% #6 12179 Microsoft   5.263
% #7 3143439  Twitter  4.766
% #8 1521427  YouTube  4.666
% #9 170062   ARPANET  4.517
%
% ---
% Parameters
% Algorihtm   Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Internet
% alpha 0.3
%
% Ranking
%    ID Label Score
% #0 9167  Internet 0.700
% #1 49488 Voice over IP  0.001
% #2 9790  Internet protocol suite 0.001
% #3 190613   Internet forum 0.001
% #4 193939   Internet access   0.001
% #5 66908 Internet service provider  0.001
% #6 6013  Email 0.001
% #7 8293  HTML  0.001
% #8 8448  Hypertext Transfer Protocol   0.001
% #9 107465   Virtual private network 0.001
%
% ---
% Parameters
% Algorihtm   Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Freddie Mercury
% maxloop  3
% scoring_function  exp
%
% Ranking
%    ID Label Score
% #0 27997 Freddie Mercury   110.259
% #1 27965 Queen (band)   13.777
% #2 27998 Brian May   6.409
% #3 129549   Roger Taylor (Queen drummer)  4.716
% #4 3317009  John Deacon 3.521
% #5 421465   Made in Heaven 3.371
% #6 1299197  We Will Rock You (musical) 3.172
% #7 1969635  Elton John  3.123
% #8 28369 The Freddie Mercury Tribute Concert 3.073
% #9 27930 Bohemian Rhapsody 3.023
%
% ---
% Parameters
% Algorihtm   Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Freddie Mercury
% alpha 0.3
%
% Ranking
%    ID Label Score
% #0 27997 Freddie Mercury   0.701
% #1 27965 Queen (band)   0.001
% #2 28369 The Freddie Mercury Tribute Concert 0.001
% #3 1975143  HIV/AIDS 0.001
% #4 338990   Queen II 0.001
% #5 123094   Mercury Phoenix Trust   0.001
% #6 107778   Middlesex   0.001
% #7 29034 Parsi 0.001
% #8 22157 Zoroastrianism 0.001
% #9 1621839  Good Old-Fashioned Lover Boy  0.001
%
% ---
% Parameters
% Algorihtm   Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Pasta
% maxloop  3
% scoring_function  exp
%
% Ranking
%    ID Label Score
% #0 15499 Pasta 29.886
% #1 1592723  Italian cuisine   4.019
% #2 9162  Italy 2.326
% #3 19009 Spaghetti   1.828
% #4 37169 Flour 1.380
% #5 234712   Durum 1.131
% #6 213678   Dough 1.032
% #7 24172 Wheat 0.996
% #8 266440   Carbonara   0.982
% #9 18082 Starch   0.932
%
% ---
% Parameters
% Algorihtm   Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Pasta
% alpha 0.3
%
% Ranking
%    ID Label Score
% #0 15499 Pasta 0.701
% #1 8059824  Bolognese sauce   0.002
% #2 266440   Carbonara   0.002
% #3 234712   Durum 0.002
% #4 9162  Italy 0.002
% #5 1493367  United States  0.002
% #6 18018 Sicily   0.002
% #7 29802 Apulia   0.002
% #8 37169 Flour 0.002
% #9 1592723  Italian cuisine   0.002
%

==> tables/comparison_wikipedia-cr3-pr0_3-ssppr0_3.tex <==
\resizebox{.95\textwidth}{!}{
\begin{tabular}{@{}rp{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}@{}}
  \toprule
    \textbf{page}
  & \multicolumn{2}{c}{\thead{\bfseries Internet}}%
  & \multicolumn{2}{c}{\thead{\bfseries Freddie Mercury}}%
  & \multicolumn{2}{c}{\thead{\bfseries Pasta}}%
  \\ %
  \cmidrule(l){2-3}%
  \cmidrule(l){4-5}%
  \cmidrule(l){6-7}%
  %
    \textbf{\#}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Pers.PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Pers.PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Pers.PageRank}}%
  \\%
  1  & Internet                                     & Internet                                           %
     & Freddie Mercury                              & Freddie Mercury                                    %
     & Pasta                                        & Pasta                                              %
     \\%
  2  & \makecell[tl]{Index of Internet-related\\%
                     articles}                      & Voice over IP                                      %
     & Queen (band)                                 & Queen (band)                                       %
     & Italian cuisine                              & Bolognese sauce                                    %
     \\%
  3  & Computer network                             & Internet protocol suite                            %
     & Brian May                                    & \makecell[tl]{The Freddie Mercury\\%
                                                                    Tribute Concert}                     %
     & Italy                                        & Carbonara                                          %
     \\%
  4  & Facebook                                     & Internet forum                                     %
     & \makecell[tl]{Roger Taylor\\%
                     (Queen drummer)}               & HIV/AIDS                                           %
     & Spaghetti                                    & Durum                                              %
     \\%
  5  & World Wide Web                               & Internet access                                    %
     & John Deacon                                  & Queen II                                           %
     & Flour                                        & Italy                                              %
     \\%
  6  & Google                                       & Internet service provider                          %
     & Made in Heaven                               & Mercury Phoenix Trust                              %
     & Durum                                        & United States                                      %
     \\%
  7  & Microsoft                                    & Email                                              %
     & \makecell[tl]{We Will Rock You\\%
                     (musical)}                     & Middlesex                                          %
     & Dough                                        & Sicily                                             %
     \\%
  8  & Twitter                                      & HTML                                               %
     & Elton John                                   & Parsi                                              %
     & Wheat                                        & Apulia                                             %
     \\%
  9  & YouTube                                      & \makecell[tl]{Hypertext Transfer\\ Protocol}       %
     & \makecell[tl]{The Freddie Mercury\\%
                     Tribute Concert}               & Zoroastrianism                                     %
     & Carbonara                                    & Flour                                              %
     \\%
  10 & ARPANET                                      & Virtual private network                            %
     & Bohemian Rhapsody                            & \makecell[tl]{Good Old-Fashioned\\
                                                                    Lover Boy}                           %
     & Starch                                       & Italian cuisine                                    %
     \\%
  \bottomrule
\end{tabular}%
}

% ---
% Parameters
% Algorihtm   Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Internet
% maxloop  3
% scoring_function  exp
%
% Ranking
%    ID Label Score
% #0 9167  Internet 298.056
% #1 151847   Index of Internet-related articles  7.852
% #2 1705417  Computer network  6.558
% #3 2614687  Facebook 5.911
% #4 21479 World Wide Web 5.562
% #5 611580   Google   5.512
% #6 12179 Microsoft   5.263
% #7 3143439  Twitter  4.766
% #8 1521427  YouTube  4.666
% #9 170062   ARPANET  4.517
%
% ---
% Parameters
% Algorihtm   Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Internet
% alpha 0.3
%
% Ranking
%    ID Label Score
% #0 9167  Internet 0.700
% #1 49488 Voice over IP  0.001
% #2 9790  Internet protocol suite 0.001
% #3 190613   Internet forum 0.001
% #4 193939   Internet access   0.001
% #5 66908 Internet service provider  0.001
% #6 6013  Email 0.001
% #7 8293  HTML  0.001
% #8 8448  Hypertext Transfer Protocol   0.001
% #9 107465   Virtual private network 0.001
%
% ---
% Parameters
% Algorihtm   Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Freddie Mercury
% maxloop  3
% scoring_function  exp
%
% Ranking
%    ID Label Score
% #0 27997 Freddie Mercury   110.259
% #1 27965 Queen (band)   13.777
% #2 27998 Brian May   6.409
% #3 129549   Roger Taylor (Queen drummer)  4.716
% #4 3317009  John Deacon 3.521
% #5 421465   Made in Heaven 3.371
% #6 1299197  We Will Rock You (musical) 3.172
% #7 1969635  Elton John  3.123
% #8 28369 The Freddie Mercury Tribute Concert 3.073
% #9 27930 Bohemian Rhapsody 3.023
%
% ---
% Parameters
% Algorihtm   Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Freddie Mercury
% alpha 0.3
%
% Ranking
%    ID Label Score
% #0 27997 Freddie Mercury   0.701
% #1 27965 Queen (band)   0.001
% #2 28369 The Freddie Mercury Tribute Concert 0.001
% #3 1975143  HIV/AIDS 0.001
% #4 338990   Queen II 0.001
% #5 123094   Mercury Phoenix Trust   0.001
% #6 107778   Middlesex   0.001
% #7 29034 Parsi 0.001
% #8 22157 Zoroastrianism 0.001
% #9 1621839  Good Old-Fashioned Lover Boy  0.001
%
% ---
% Parameters
% Algorihtm   Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Pasta
% maxloop  3
% scoring_function  exp
%
% Ranking
%    ID Label Score
% #0 15499 Pasta 29.886
% #1 1592723  Italian cuisine   4.019
% #2 9162  Italy 2.326
% #3 19009 Spaghetti   1.828
% #4 37169 Flour 1.380
% #5 234712   Durum 1.131
% #6 213678   Dough 1.032
% #7 24172 Wheat 0.996
% #8 266440   Carbonara   0.982
% #9 18082 Starch   0.932
%
% ---
% Parameters
% Algorihtm   Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source   Pasta
% alpha 0.3
%
% Ranking
%    ID Label Score
% #0 15499 Pasta 0.701
% #1 8059824  Bolognese sauce   0.002
% #2 266440   Carbonara   0.002
% #3 234712   Durum 0.002
% #4 9162  Italy 0.002
% #5 1493367  United States  0.002
% #6 18018 Sicily   0.002
% #7 29802 Apulia   0.002
% #8 37169 Flour 0.002
% #9 1592723  Italian cuisine   0.002
%

==> tables/comparison_wikipedia-cr3-pr0_85-ssppr0_85-top5.tex <==
\resizebox{.95\textwidth}{!}{
  \begin{tabular}{@{}rp{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}@{}}
  \toprule
    \textbf{page}
  & \multicolumn{2}{c}{\thead{\bfseries Internet}}%
  & \multicolumn{2}{c}{\thead{\bfseries Freddie Mercury}}%
  & \multicolumn{2}{c}{\thead{\bfseries Pasta}}%
  \\ %
  \cmidrule(l){2-3}%
  \cmidrule(l){4-5}%
  \cmidrule(l){6-7}%
  %
    \textbf{\#}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  \\%
  1  & Internet                                     & Internet                                            %
     & Freddie Mercury                              & Freddie Mercury                                     %
     & Pasta                                        & Pasta                                               %
     \\%
  2  & \makecell[t,l]{Index of Internet-related \\%
                      articles}                     & Voice over IP                                       %
     & Queen (band)                                 & Queen (band)                                        %
     & Italian cuisine                              & Italy                                               %
     \\%
  3  & Computer network                             & United States                                       %
     & Brian May                                    & London                                              %
     & Italy                                        & United States                                       %
     \\%
  4  & Facebook                                     & Internet protocol suite                             %
     & \makecell[t,l]{Roger Taylor \\               %
                      (Queen drummer)}              & United States                                       %
     & Spaghetti                                    & Bolognese sauce                                     %
     \\%
  5  & World Wide Web                               & \makecell[t,l]{Internet Engineering \\              %
                                                                     Task Force}                          %
     & John Deacon                                  & HIV/AIDS                                            %
     & Flour                                        & Durum                                               %
     \\%
  \bottomrule
\end{tabular}%
}

% ---
% Parameters
% Algorihtm  Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Internet
% maxloop  3
% scoring_function  exp
%
% Ranking
%   ID  Label  Score
% #0  9167  Internet  298.056
% #1  151847  Index of Internet-related articles  7.852
% #2  1705417  Computer network  6.558
% #3  2614687  Facebook  5.911
% #4  21479  World Wide Web  5.562
% #5  611580  Google  5.512
% #6  12179  Microsoft  5.263
% #7  3143439  Twitter  4.766
% #8  1521427  YouTube  4.666
% #9  170062  ARPANET  4.517
%
% ---
% Parameters
% Algorihtm  Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Internet
% alpha  0.85
%
% Ranking
%   ID  Label  Score
% #0  9167  Internet  0.152
% #1  49488  Voice over IP  0.001
% #2  1493367  United States  0.001
% #3  9790  Internet protocol suite  0.001
% #4  9661  Internet Engineering Task Force  0.001
% #5  19948  The New York Times  0.001
% #6  1705417  Computer network  0.001
% #7  190613  Internet forum  0.001
% #8  193939  Internet access  0.001
% #9  66908  Internet service provider  0.001
%
% Parameters
% Algorihtm  Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Freddie Mercury
% maxloop  3
% scoring_function  exp
%
% Ranking
%   ID  Label  Score
% #0  27997  Freddie Mercury  110.259
% #1  27965  Queen (band)  13.777
% #2  27998  Brian May  6.409
% #3  129549  Roger Taylor (Queen drummer)  4.716
% #4  3317009  John Deacon  3.521
% #5  421465  Made in Heaven  3.371
% #6  1299197  We Will Rock You (musical)  3.172
% #7  1969635  Elton John  3.123
% #8  28369  The Freddie Mercury Tribute Concert  3.073
% #9  27930  Bohemian Rhapsody  3.023
%
% ---
% Parameters
% Algorihtm  Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Freddie Mercury
% alpha  0.85
%
% Ranking
%   ID  Label  Score
% #0  27997  Freddie Mercury  0.151
% #1  27965  Queen (band)  0.001
% #2  11414  London  0.001
% #3  1493367  United States  0.001
% #4  1975143  HIV/AIDS  0.001
% #5  16579  Rock music  0.001
% #6  28369  The Freddie Mercury Tribute Concert  0.001
% #7  129549  Roger Taylor (Queen drummer)  0.001
% #8  20613  United Kingdom  0.001
% #9  5334347  BBC  0.001
%
% ---
% Parameters
% Algorihtm Cyclerank
% Dataset enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Pasta
% maxloop 3
% scoring_function  exp
%
% Ranking
%   ID  Label Score
% #0  15499 Pasta 29.886
% #1  1592723 Italian cuisine 4.019
% #2  9162  Italy 2.326
% #3  19009 Spaghetti 1.828
% #4  37169 Flour 1.380
% #5  234712  Durum 1.131
% #6  213678  Dough 1.032
% #7  24172 Wheat 0.996
% #8  266440  Carbonara 0.982
% #9  18082 Starch  0.932
%
% ---
% Parameters
% Algorihtm Single Source Personalized PageRank
% Dataset enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Pasta
% alpha 0.85
%
% Ranking
%   ID  Label Score
% #0  15499 Pasta 0.152
% #1  9162  Italy 0.003
% #2  1493367 United States 0.002
% #3  8059824 Bolognese sauce 0.002
% #4  234712  Durum 0.002
% #5  266440  Carbonara 0.002
% #6  11298 Latin 0.001
% #7  16602 Rome  0.001
% #8  9266  Italian language  0.001
% #9  9849  Japan 0.001
%

==> tables/comparison_wikipedia-cr3-pr0_85-ssppr0_85.tex <==
\resizebox{.95\textwidth}{!}{
  \begin{tabular}{@{}rp{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}@{}}
  \toprule
    \textbf{page}
  & \multicolumn{2}{c}{\thead{\bfseries Internet}}%
  & \multicolumn{2}{c}{\thead{\bfseries Freddie Mercury}}%
  & \multicolumn{2}{c}{\thead{\bfseries Pizza}}%
  \\ %
  \cmidrule(l){2-3}%
  \cmidrule(l){4-5}%
  \cmidrule(l){6-7}%
  %
    \textbf{\#}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  \\%
  1  & Internet                                     & Internet                                            %
     & Freddie Mercury                              & Freddie Mercury                                     %
     & Pasta                                        & Pasta                                               %
     \\%
  2  & \makecell[tl]{Index of Internet-related\\%
                     articles}                      & Voice over IP                                       %
     & Queen (band)                                 & Queen (band)                                        %
     & Italian cuisine                              & Italy                                               %
     \\%
  3  & Computer network                             & United States                                       %
     & Brian May                                    & London                                              %
     & Italy                                        & United States                                       %
     \\%
  4  & Facebook                                     & Internet protocol suite                             %
     & \makecell[tl]{Roger Taylor\\%
                     (Queen drummer)}               & United States                                       %
     & Spaghetti                                    & Bolognese sauce                                     %
     \\%
  5  & World Wide Web                               & \makecell[tl]{Internet Engineering \\               %
                                                                    Task Force}                           %
     & John Deacon                                  & HIV/AIDS                                            %
     & Flour                                        & Durum                                               %
     \\%
  6  & Google                                       & The New York Times                                  %
     & Made in Heaven                               & Rock music                                          %
     & Durum                                        & Carbonara                                           %
     \\%
  7  & Microsoft                                    & Computer network                                    %
     & \makecell[tl]{We Will Rock You\\%
                     (musical)}                     & \makecell[tl]{The Freddie Mercury\\%
                                                                    Tribute Concert}                      %
     & Dough                                        & Latin                                               %
     \\%
  8  & Twitter                                      & Internet forum                                      %
     & Elton John                                   & \makecell[tl]{Roger Taylor\\%
                                                                    (Queen drummer)}                      %
     & Wheat                                        & Rome                                                %
     \\%
  9  & YouTube                                      & Internet access                                     %
     & \makecell[tl]{The Freddie Mercury\\%
                     Tribute Concert}               & United Kingdom                                      %
     & Carbonara                                    & Italian language                                    %
     \\%
  10 & ARPANET                                      & Internet service provider                           %
     & Bohemian Rhapsody                            & BBC                                                 %
     & Starch                                       & Japan                                               %
     \\%
  \bottomrule
\end{tabular}%
}

% ---
% Parameters
% Algorihtm  Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Internet
% maxloop  3
% scoring_function  exp
%
% Ranking
%   ID  Label  Score
% #0  9167  Internet  298.056
% #1  151847  Index of Internet-related articles  7.852
% #2  1705417  Computer network  6.558
% #3  2614687  Facebook  5.911
% #4  21479  World Wide Web  5.562
% #5  611580  Google  5.512
% #6  12179  Microsoft  5.263
% #7  3143439  Twitter  4.766
% #8  1521427  YouTube  4.666
% #9  170062  ARPANET  4.517
%
% ---
% Parameters
% Algorihtm  Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Internet
% alpha  0.85
%
% Ranking
%   ID  Label  Score
% #0  9167  Internet  0.152
% #1  49488  Voice over IP  0.001
% #2  1493367  United States  0.001
% #3  9790  Internet protocol suite  0.001
% #4  9661  Internet Engineering Task Force  0.001
% #5  19948  The New York Times  0.001
% #6  1705417  Computer network  0.001
% #7  190613  Internet forum  0.001
% #8  193939  Internet access  0.001
% #9  66908  Internet service provider  0.001
%
% Parameters
% Algorihtm  Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Freddie Mercury
% maxloop  3
% scoring_function  exp
%
% Ranking
%   ID  Label  Score
% #0  27997  Freddie Mercury  110.259
% #1  27965  Queen (band)  13.777
% #2  27998  Brian May  6.409
% #3  129549  Roger Taylor (Queen drummer)  4.716
% #4  3317009  John Deacon  3.521
% #5  421465  Made in Heaven  3.371
% #6  1299197  We Will Rock You (musical)  3.172
% #7  1969635  Elton John  3.123
% #8  28369  The Freddie Mercury Tribute Concert  3.073
% #9  27930  Bohemian Rhapsody  3.023
%
% ---
% Parameters
% Algorihtm  Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Freddie Mercury
% alpha  0.85
%
% Ranking
%   ID  Label  Score
% #0  27997  Freddie Mercury  0.151
% #1  27965  Queen (band)  0.001
% #2  11414  London  0.001
% #3  1493367  United States  0.001
% #4  1975143  HIV/AIDS  0.001
% #5  16579  Rock music  0.001
% #6  28369  The Freddie Mercury Tribute Concert  0.001
% #7  129549  Roger Taylor (Queen drummer)  0.001
% #8  20613  United Kingdom  0.001
% #9  5334347  BBC  0.001
%
% ---
% Parameters
% Algorihtm Cyclerank
% Dataset enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Pasta
% maxloop 3
% scoring_function  exp
%
% Ranking
%   ID  Label Score
% #0  15499 Pasta 29.886
% #1  1592723 Italian cuisine 4.019
% #2  9162  Italy 2.326
% #3  19009 Spaghetti 1.828
% #4  37169 Flour 1.380
% #5  234712  Durum 1.131
% #6  213678  Dough 1.032
% #7  24172 Wheat 0.996
% #8  266440  Carbonara 0.982
% #9  18082 Starch  0.932
%
% ---
% Parameters
% Algorihtm Single Source Personalized PageRank
% Dataset enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Pasta
% alpha 0.85
%
% Ranking
%   ID  Label Score
% #0  15499 Pasta 0.152
% #1  9162  Italy 0.003
% #2  1493367 United States 0.002
% #3  8059824 Bolognese sauce 0.002
% #4  234712  Durum 0.002
% #5  266440  Carbonara 0.002
% #6  11298 Latin 0.001
% #7  16602 Rome  0.001
% #8  9266  Italian language  0.001
% #9  9849  Japan 0.001
%

==> tables/comparison_wikipedia-cr4-pr0_85-ssppr0_85-top5.tex <==
 \resizebox{.95\textwidth}{!}{
  \begin{tabular}{@{}rp{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}@{}}
  \toprule
    \textbf{page}
  & \multicolumn{2}{c}{\thead{\bfseries Internet}}%
  & \multicolumn{2}{c}{\thead{\bfseries Freddie Mercury}}%
  & \multicolumn{2}{c}{\thead{\bfseries Pasta}}%
  \\ %
  \cmidrule(l){2-3}%
  \cmidrule(l){4-5}%
  \cmidrule(l){6-7}%
  %
    \textbf{\#}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  \\%
  1  & Internet                                     & Internet                                            %
     & Freddie Mercury                              & Freddie Mercury                                     %
     & Pasta                                        & Pasta                                               %
     \\%
  2  & 2a                                           & Voice over IP                                       %
     & 2b                                 & Queen (band)                                        %
     & 2c                              & Italy                                               %
     \\%
  3  & 3a                             & United States                                       %
     & 3b                                    & London                                              %
     & 3c                                        & United States                                       %
     \\%
  4  & 4a                                     & Internet protocol suite                             %
     & 4b               & United States                                       %
     & 4c                                    & Bolognese sauce                                     %
     \\%
  5  & 5a                               & \makecell[tl]{Internet Engineering \\               %
                                                                    Task Force}                           %
     & 5b                                  & HIV/AIDS                                            %
     & 5c                                        & Durum                                               %
     \\%
  \bottomrule
\end{tabular}%
}

% ---
% Parameters
% Algorihtm  Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Internet
% maxloop  3
% scoring_function  exp
%
% Ranking
%   ID  Label  Score
% #0  9167  Internet  298.056
% #1  151847  Index of Internet-related articles  7.852
% #2  1705417  Computer network  6.558
% #3  2614687  Facebook  5.911
% #4  21479  World Wide Web  5.562
% #5  611580  Google  5.512
% #6  12179  Microsoft  5.263
% #7  3143439  Twitter  4.766
% #8  1521427  YouTube  4.666
% #9  170062  ARPANET  4.517
%
% ---
% Parameters
% Algorihtm  Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Internet
% alpha  0.85
%
% Ranking
%   ID  Label  Score
% #0  9167  Internet  0.152
% #1  49488  Voice over IP  0.001
% #2  1493367  United States  0.001
% #3  9790  Internet protocol suite  0.001
% #4  9661  Internet Engineering Task Force  0.001
% #5  19948  The New York Times  0.001
% #6  1705417  Computer network  0.001
% #7  190613  Internet forum  0.001
% #8  193939  Internet access  0.001
% #9  66908  Internet service provider  0.001
%
% Parameters
% Algorihtm  Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Freddie Mercury
% maxloop  3
% scoring_function  exp
%
% Ranking
%   ID  Label  Score
% #0  27997  Freddie Mercury  110.259
% #1  27965  Queen (band)  13.777
% #2  27998  Brian May  6.409
% #3  129549  Roger Taylor (Queen drummer)  4.716
% #4  3317009  John Deacon  3.521
% #5  421465  Made in Heaven  3.371
% #6  1299197  We Will Rock You (musical)  3.172
% #7  1969635  Elton John  3.123
% #8  28369  The Freddie Mercury Tribute Concert  3.073
% #9  27930  Bohemian Rhapsody  3.023
%
% ---
% Parameters
% Algorihtm  Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Freddie Mercury
% alpha  0.85
%
% Ranking
%   ID  Label  Score
% #0  27997  Freddie Mercury  0.151
% #1  27965  Queen (band)  0.001
% #2  11414  London  0.001
% #3  1493367  United States  0.001
% #4  1975143  HIV/AIDS  0.001
% #5  16579  Rock music  0.001
% #6  28369  The Freddie Mercury Tribute Concert  0.001
% #7  129549  Roger Taylor (Queen drummer)  0.001
% #8  20613  United Kingdom  0.001
% #9  5334347  BBC  0.001
%
% ---
% Parameters
% Algorihtm Cyclerank
% Dataset enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Pasta
% maxloop 3
% scoring_function  exp
%
% Ranking
%   ID  Label Score
% #0  15499 Pasta 29.886
% #1  1592723 Italian cuisine 4.019
% #2  9162  Italy 2.326
% #3  19009 Spaghetti 1.828
% #4  37169 Flour 1.380
% #5  234712  Durum 1.131
% #6  213678  Dough 1.032
% #7  24172 Wheat 0.996
% #8  266440  Carbonara 0.982
% #9  18082 Starch  0.932
%
% ---
% Parameters
% Algorihtm Single Source Personalized PageRank
% Dataset enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Pasta
% alpha 0.85
%
% Ranking
%   ID  Label Score
% #0  15499 Pasta 0.152
% #1  9162  Italy 0.003
% #2  1493367 United States 0.002
% #3  8059824 Bolognese sauce 0.002
% #4  234712  Durum 0.002
% #5  266440  Carbonara 0.002
% #6  11298 Latin 0.001
% #7  16602 Rome  0.001
% #8  9266  Italian language  0.001
% #9  9849  Japan 0.001
%

==> tables/comparison_wikipedia-cr4-pr0_85-ssppr0_85.tex <==
 \resizebox{.95\textwidth}{!}{
  \begin{tabular}{@{}rp{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}p{2.75cm}@{}}
  \toprule
    \textbf{page}
  & \multicolumn{2}{c}{\thead{\bfseries Internet}}%
  & \multicolumn{2}{c}{\thead{\bfseries Freddie Mercury}}%
  & \multicolumn{2}{c}{\thead{\bfseries Pasta}}%
  \\ %
  \cmidrule(l){2-3}%
  \cmidrule(l){4-5}%
  \cmidrule(l){6-7}%
  %
    \textbf{\#}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  & \multicolumn{1}{c}{\thead{\bfseries Cyclerank}} & \multicolumn{1}{c}{\thead{\bfseries Personalized PageRank}}%
  \\%
  1  & Internet                                     & Internet                                            %
     & Freddie Mercury                              & Freddie Mercury                                     %
     & Pasta                                        & Pasta                                               %
     \\%
  2  & 2a                                           & Voice over IP                                       %
     & 2b                                 & Queen (band)                                        %
     & 2c                              & Italy                                               %
     \\%
  3  & 3a                             & United States                                       %
     & 3b                                    & London                                              %
     & 3c                                        & United States                                       %
     \\%
  4  & 4a                                     & Internet protocol suite                             %
     & 4b               & United States                                       %
     & 4c                                    & Bolognese sauce                                     %
     \\%
  5  & 5a                               & \makecell[tl]{Internet Engineering \\               %
                                                                    Task Force}                           %
     & 5b                                  & HIV/AIDS                                            %
     & 5c                                        & Durum                                               %
     \\%
  6  & 6a                                       & The New York Times                                  %
     & 6b                               & Rock music                                          %
     & 6c                                        & Carbonara                                           %
     \\%
  7  & 7a                                    & Computer network                                    %
     & 7b                     & \makecell[tl]{The Freddie Mercury\\%
                                                                    Tribute Concert}                      %
     & 7c                                        & Latin                                               %
     \\%
  8  & 8a                                      & Internet forum                                      %
     & 8b                                   & \makecell[tl]{Roger Taylor\\%
                                                                    (Queen drummer)}                      %
     & 8c                                        & Rome                                                %
     \\%
  9  & 9a                                      & Internet access                                     %
     & 9b               & United Kingdom                                      %
     & 9c                                    & Italian language                                    %
     \\%
  10 & 10a                                      & Internet service provider                           %
     & 10b                            & BBC                                                 %
     & 10c                                       & Japan                                               %
     \\%
  \bottomrule
\end{tabular}%
}

% ---
% Parameters
% Algorihtm  Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Internet
% maxloop  3
% scoring_function  exp
%
% Ranking
%   ID  Label  Score
% #0  9167  Internet  298.056
% #1  151847  Index of Internet-related articles  7.852
% #2  1705417  Computer network  6.558
% #3  2614687  Facebook  5.911
% #4  21479  World Wide Web  5.562
% #5  611580  Google  5.512
% #6  12179  Microsoft  5.263
% #7  3143439  Twitter  4.766
% #8  1521427  YouTube  4.666
% #9  170062  ARPANET  4.517
%
% ---
% Parameters
% Algorihtm  Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Internet
% alpha  0.85
%
% Ranking
%   ID  Label  Score
% #0  9167  Internet  0.152
% #1  49488  Voice over IP  0.001
% #2  1493367  United States  0.001
% #3  9790  Internet protocol suite  0.001
% #4  9661  Internet Engineering Task Force  0.001
% #5  19948  The New York Times  0.001
% #6  1705417  Computer network  0.001
% #7  190613  Internet forum  0.001
% #8  193939  Internet access  0.001
% #9  66908  Internet service provider  0.001
%
% Parameters
% Algorihtm  Cyclerank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Freddie Mercury
% maxloop  3
% scoring_function  exp
%
% Ranking
%   ID  Label  Score
% #0  27997  Freddie Mercury  110.259
% #1  27965  Queen (band)  13.777
% #2  27998  Brian May  6.409
% #3  129549  Roger Taylor (Queen drummer)  4.716
% #4  3317009  John Deacon  3.521
% #5  421465  Made in Heaven  3.371
% #6  1299197  We Will Rock You (musical)  3.172
% #7  1969635  Elton John  3.123
% #8  28369  The Freddie Mercury Tribute Concert  3.073
% #9  27930  Bohemian Rhapsody  3.023
%
% ---
% Parameters
% Algorihtm  Single Source Personalized PageRank
% Dataset  enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Freddie Mercury
% alpha  0.85
%
% Ranking
%   ID  Label  Score
% #0  27997  Freddie Mercury  0.151
% #1  27965  Queen (band)  0.001
% #2  11414  London  0.001
% #3  1493367  United States  0.001
% #4  1975143  HIV/AIDS  0.001
% #5  16579  Rock music  0.001
% #6  28369  The Freddie Mercury Tribute Concert  0.001
% #7  129549  Roger Taylor (Queen drummer)  0.001
% #8  20613  United Kingdom  0.001
% #9  5334347  BBC  0.001
%
% ---
% Parameters
% Algorihtm Cyclerank
% Dataset enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Pasta
% maxloop 3
% scoring_function  exp
%
% Ranking
%   ID  Label Score
% #0  15499 Pasta 29.886
% #1  1592723 Italian cuisine 4.019
% #2  9162  Italy 2.326
% #3  19009 Spaghetti 1.828
% #4  37169 Flour 1.380
% #5  234712  Durum 1.131
% #6  213678  Dough 1.032
% #7  24172 Wheat 0.996
% #8  266440  Carbonara 0.982
% #9  18082 Starch  0.932
%
% ---
% Parameters
% Algorihtm Single Source Personalized PageRank
% Dataset enwiki.wikigraph.2018-03-01.cleaned.csv
% Source  Pasta
% alpha 0.85
%
% Ranking
%   ID  Label Score
% #0  15499 Pasta 0.152
% #1  9162  Italy 0.003
% #2  1493367 United States 0.002
% #3  8059824 Bolognese sauce 0.002
% #4  234712  Durum 0.002
% #5  266440  Carbonara 0.002
% #6  11298 Latin 0.001
% #7  16602 Rome  0.001
% #8  9266  Italian language  0.001
% #9  9849  Japan 0.001
%
